Sequential Neural Barriers for Scalable Dynamic Obstacle Avoidance

There are two major challenges for scaling up robot navigation around dynamic obstacles: the complex interaction dynamics of the obstacles can be hard to model analytically, and the complexity of planning and control grows exponentially in the number of obstacles. Data-driven and learning-based methods are thus particularly valuable in this context. However, data-driven methods are sensitive to distribution drift, making it hard to train and generalize learned models across different obstacle densities. We propose a novel method for compositional learning of Sequential Neural Control Barrier models (SNCBFs) to achieve scalability. Our approach exploits an important observation: the spatial interaction patterns of multiple dynamic obstacles can be decomposed and predicted through temporal sequences of states for each obstacle. Through decomposition, we can generalize control policies trained only with a small number of obstacles, to environments where the obstacle density can be 100x higher. We demonstrate the benefits of the proposed methods in improving dynamic collision avoidance in comparison with existing methods including potential fields, end-to-end reinforcement learning, and model-predictive control. We also perform hardware experiments and show the practical effectiveness of the approach in the supplementary video.

==> NOTES <==
important papers to cite: 

http://ames.caltech.edu/2016CDC_Composable_Barrier_Final.pdf

https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7857061 analytic methods for constructing compositional barriers

https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=7937882 Nonsmooth Barrier Functions With Applications to Multi-Robot Systems

https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8511471 Boolean composition continued

https://arxiv.org/abs/2201.01347 "generalization" of control barriers but in a different context

https://www.diva-portal.org/smash/get/diva2:1457693/FULLTEXT01.pdf
https://arxiv.org/abs/2010.10190


\citet{DBLP:conf/cdc/WangAE16} composes the CBF for a team of mobile robots by designing the piecewise barrier function based on a connectivity distance. Further, \citet{DBLP:journals/trob/WangAE17} gives an analytic method to construct the compositional barriers. \citet{DBLP:journals/csysl/GlotfelterCE17} extends the analysis of barrier function to a class of nonsmooth barrier functions, which enables the use of max and min operators. \citet{DBLP:conf/ccta/GlotfelterCE18} extends the Boolean composition of nonsmooth barrier functions to nonsmooth control barrier functions, by explicitly addressing the controlled systems. \citet{ma2022learning} focuses the generazation of control barrier functions to various configurations of static obstacles, while our approach focuses the generalization for scalable dynamic obstacles.

==> list_of_variables.tex <==
state: $x \in D\subseteq \mathbb R^n $
time: $t$
dynamics: $f(x(t), u(t))$
control: $u(t)\in U\subseteq \mathbb{R}^p$


unsafe set in ego-agent state space: $X_u \in X$
forward invariant set in ego-agent state space: $I \in X$


CBF: $B: \mathbb{R}^n \rightarrow \mathbb{R}$
zero-superlevel set: $\mathcal{C} \subseteq X$
class k function: $\alpha$
maximal discount rate: $\lambda$
lipchitz continuous controller: $u(x) = K_{\text{cbf}}$

implicit parameter space: $H\subseteq \mathbb{R}^{k\times m}$
encoded vector concatenated from LSTM and MLP: $d$

safe set: $D_s\subseteq X\times H$ 
unsafe set: $D_u\subseteq X\times H$ 

loss function: $L_{B,D}$
error margin: $\phi_{\gamma}$

discrete transitions: $\Delta t$ is the time needed to travel from $(x,h)$ to $(x',h')$
state transitions for ego-agent: $\pi: X \times U \rightarrow X$,

threshold safety parameter: $\theta$
critical samples $D^{\theta}=\{(x,h) \in D_s\cup D_u: B(x,h) \in [0,\theta]\}$

number of obstacles in environment: $q$

threshold for aggregating obstacles: $b$
sequence of relative states of an obstacle $i$: $h_i$
aggregate CBF: $\hat B(x)$

candidate control actions in alg 2: $u_1,...,u_l$
